Long-term spin-down and low luminosity regime in the Be/X-ray binary pulsar GX 304-1

We carry out timing and spectral studies of the Be/X-ray binary pulsar GX 304-1 using NuStar and XMM-Newton observations. We construct the long-term spin period evolution of the pulsar which changes from a long-term spin-up ($\sim 1.3 \times 10^{-13} $Hz \~s$^{-1}$) to a long-term spin-down ($\sim -3.4 \times 10^{-14} $Hz \~s$^{-1}$) trend during a low luminosity state ($\sim 10^{34-35} $erg \~s$^{-1}$). A prolonged low luminosity regime ($L_X \sim 10^{34-35} $erg \~s$^{-1}$) was detected during 2005-2010 and spanning nearly five years since 2018 December. The XMM-Newton and NuStar spectra can be described with a power law plus blackbody model having an estimated luminosity of $\sim 2.5 \times 10^{33} $erg \~s$^{-1}$ and $\sim 3.6 \times 10^{33} $erg \~s$^{-1}$ respectively. The inferred radius of the blackbody emission is about 100-110 m which suggests a polar-cap origin of this component. From long-term ultraviolet observations of the companion star, an increase in the ultraviolet signatures is detected preceding the X-ray outbursts. The spectral energy distribution of the companion star is constructed which provides a clue of possible UV excess when X-ray outbursts were detected from the neutron star compared to the quiescent phase. We explore plausible mechanisms to explain the long-term spin-down and extended low luminosity manifestation in this pulsar. We find that sustained accretion from a cold disc may explain the prolonged low luminosity state of the pulsar since December 2018 but the pulsar was undergoing normal accretion during the low luminosity period spanning 2005-2010.

==> authors.tex <==
\author{Z.~Wang (\begin{CJK*}{UTF8}{gbsn}王子腾\end{CJK*})}
\affiliation{International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}

\author{K.~W.~Bannister}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{V.~Gupta}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{X.~Deng}
\affiliation{The 54th Institute of China Electronics Technology Group Corporation, 580 Zhongshan W Rd, Shijiazhuang 050002, Hebei, China}
\alsoaffiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{M.~Pilawa}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{J.~Tuthill}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

%%%%%%% main craco commissioner and developer

\author{J.~D.~Bunton}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{C.~Flynn}
\affiliation{Center for Astrophysics and Supercomputing, Swinburne University of Technology, Post Office Box 218, Hawthorn, VIC 3122, Australia}
\alsoaffiliation{ARC Centre of Excellence for Gravitational Wave Discovery (OzGrav), Post Office Box 218, Hawthorn, VIC 3122, Australia}

\author{M.~Glowacki}
\affiliation{International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}

\author{A.~Jaini}
\affiliation{Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}

\author{Y.~W.~J.~Lee}
\affiliation{Sydney Institute for Astronomy, School of Physics, The University of Sydney, Sydney, 2006, NSW, Australia}
\alsoaffiliation{ARC Centre of Excellence for Gravitational Wave Discovery (OzGrav), Post Office Box 218, Hawthorn, VIC 3122, Australia}
\alsoaffiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{E.~Lenc}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{J.~Lucero}
% \affiliation{\todo{Advanced Micro Devices Inc, 2485 Augustine Dr, Santa Clara, CA 95054, USA}}
\affiliation{Advanced Micro Devices Inc, 2485 Augustine Dr, Santa Clara, CA 95054, USA}

\author{A.~Paek}
% \affiliation{\todo{Advanced Micro Devices Inc, 2485 Augustine Dr, Santa Clara, CA 95054, USA}}
\affiliation{Advanced Micro Devices Inc, 2485 Augustine Dr, Santa Clara, CA 95054, USA}

\author{R.~Radhakrishnan}
\affiliation{Advanced Micro Devices Inc, 2485 Augustine Dr, Santa Clara, CA 95054, USA}
\alsoaffiliation{Cadence Design Systems, Inc, 2655 Seely Ave, Ste 5, San Jose, CA 95134, USA}

\author{N.~Thyagarajan}
\affiliation{CSIRO, Space And Astronomy, PO Box 1130, Bently, WA 6102, Australia}

\author{P.~Uttarkar}
\affiliation{Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}

\author{Y.~Wang}
\affiliation{Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}
\alsoaffiliation{ARC Centre of Excellence for Gravitational Wave Discovery (OzGrav), Post Office Box 218, Hawthorn, VIC 3122, Australia}

%%%%%%% LIEF grant Co-Is and operation teams
\author{N.~D.~R.~Bhat}
\affiliation{International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}

\author{C.~W.~James}
\affiliation{International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}

\author{V.~A.~Moss}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}
\alsoaffiliation{Sydney Institute for Astronomy, School of Physics, The University of Sydney, Sydney, 2006, NSW, Australia}

\author{Tara~Murphy}
\affiliation{Sydney Institute for Astronomy, School of Physics, The University of Sydney, Sydney, 2006, NSW, Australia}
\alsoaffiliation{ARC Centre of Excellence for Gravitational Wave Discovery (OzGrav), Post Office Box 218, Hawthorn, VIC 3122, Australia}

\author{J.~E.~Reynolds}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{R.~M.~Shannon}
\affiliation{Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}

\author{L.~G.~Spitler}
\affiliation{Max Planck Institute for Radio Astronomy, Auf dem H\"{u}gel 69, 53121 Bonn, Germany}

\author{A.~Tzioumis}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

%%%%%%%%%%%%% scientific inputs
\author{M.~Caleb}
\affiliation{Sydney Institute for Astronomy, School of Physics, The University of Sydney, Sydney, 2006, NSW, Australia}

\author{A.~T.~Deller}
\affiliation{Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}
\alsoaffiliation{ARC Centre of Excellence for Gravitational Wave Discovery (OzGrav), Post Office Box 218, Hawthorn, VIC 3122, Australia}

\author{A.~C.~Gordon}
\affiliation{Center for Interdisciplinary Exploration and Research in Astrophysics (CIERA) and Department of Physics and Astronomy, Northwestern University, Evanston, IL 60208, USA}

\author{L.~Marnoch}
\affiliation{School of Mathematical and Physical Sciences, Macquarie University, NSW 2109, Australia}
\alsoaffiliation{Astrophysics and Space Technologies Research Centre, Macquarie University, Sydney, NSW 2109, Australia}
\alsoaffiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}
\alsoaffiliation{ARC Centre of Excellence for All-Sky Astrophysics in 3 Dimensions (ASTRO 3D), Sydney, Australia}

\author{S.~D.~Ryder}
\affiliation{School of Mathematical and Physical Sciences, Macquarie University, NSW 2109, Australia}
\alsoaffiliation{Astrophysics and Space Technologies Research Centre, Macquarie University, Sydney, NSW 2109, Australia}

\author{S.~Simha}
\affiliation{Center for Interdisciplinary Exploration and Research in Astrophysics (CIERA) and Department of Physics and Astronomy, Northwestern University, Evanston, IL 60208, USA}
\alsoaffiliation{Department of Astronomy and Astrophysics, University of Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA}



%%%%%%%%%% builder list opt in
\author{C.~S.~Anderson}
\affiliation{Research School of Astronomy \& Astrophysics, Australian National University, Canberra ACT, Australia 2610}

\author{L.~Ball}
\affiliation{SKA Observatory, Jodrell Bank, Lower Withington, Macclesfield, Cheshire SK11 9FT, UK}
\alsoaffiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{D.~Brodrick}
\affiliation{Advanced Instrumentation Technology Centre, Research School of Astronomy \& Astrophysics, Australian National University, Canberra, Australia}

\author{F.~R.~Cooray}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{N.~Gupta}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Post Bag 4, Ganeshkhind, Pune 411 007, India}

\author{D.~B.~Hayman}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{A.~Ng}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{S.~E.~Pearce}
\affiliation{SKA Observatory, Jodrell Bank, Lower Withington, Macclesfield, Cheshire SK11 9FT, UK}
\alsoaffiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{C.~Phillips}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{M.~A.~Voronkov}
\affiliation{CSIRO, Space And Astronomy, PO Box 76, Epping, NSW 1710, Australia}

\author{T.~Westmeier}
\affiliation{International Centre for Radio Astronomy Research, The University of Western Australia, 35 Stirling Highway, Crawley, WA 6009, Australia}

% \author{author list and order TBD}

\email[Ziteng Wang]{ziteng.wang@curtin.edu.au}
